Learning Mean-Field Equations from Particle Data Using WSINDy

We develop a weak-form sparse identification method for interacting particle systems (IPS) with the primary goals of reducing computational complexity for large particle number $N$ and offering robustness to either intrinsic or extrinsic noise. In particular, we use concepts from mean-field theory of IPS in combination with the weak-form sparse identification of nonlinear dynamics algorithm (WSINDy) to provide a fast and reliable system identification scheme for recovering the governing stochastic differential equations for an IPS when the number of particles per experiment $N$ is on the order of several thousand and the number of experiments $M$ is less than 100. This is in contrast to existing work showing that system identification for $N$ less than 100 and $M$ on the order of several thousand is feasible using strong-form methods. We prove that under some standard regularity assumptions the scheme converges with rate $\mathcal{O}(N^{-1/2})$ in the ordinary least squares setting and we demonstrate the convergence rate numerically on several systems in one and two spatial dimensions. Our examples include a canonical problem from homogenization theory (as a first step towards learning coarse-grained models), the dynamics of an attractive-repulsive swarm, and the IPS description of the parabolic-elliptic Keller-Segel model for chemotaxis.

==> preamble.tex <==
\usepackage[utf8]{inputenc}
%\usepackage[nobysame]{amsrefs}
\usepackage{
algorithmic,
amsmath,
amssymb,
amsthm,
appendix,
bm,
bbm,
caption,
color,
epsf,
enumitem,
float,
graphicx,
hyperref,
listings,
mathtools,
mathrsfs,
%mcode,
subcaption,
tikz,
titletoc,
%subfig,
url,
ulem,
xcolor
%algorithm2e
}

\setcounter{secnumdepth}{2}
\setcounter{tocdepth}{3}	
\hypersetup{
    colorlinks=true, %set true if you want colored links
    linktoc=all,     %set to all if you want both sections and subsections linked
    linkcolor=black,  %choose some color if you want links to stand out
}

\numberwithin{equation}{section}

\RequirePackage{algorithm}[0.1]
%\renewcommand{\ALG@name}{Algorithm}
\renewcommand\thealgorithm{\siamprelabel\@arabic\c@algorithm}

\if@onealgnum
\else
\numberwithin{algorithm}{section}
\fi


\tikzset{every label/.style={font=\footnotesize,inner sep=1pt}}
\DeclareCaptionFormat{myformat}{#1#2#3\hrulefill}
\captionsetup[figure]{format=myformat}

\graphicspath{{figures/}}

